Spectrophotometry of 237 stars in 7 Open Clusters

Photoelectric spectrophotometry is presented for 237 stars in the Hyades, Pleiades, Alpha Persei, Praesepe, Coma Berenices, IC~4665, and M39 open clusters. 16 bandpasses were observed from 350 nm to 778 nm, with 3.2 to 6.4 nm bandwidth. Data are standardized to the Hayes-Latham system to mutual accuracy of 0.016 mag per passband. By comparison to SIMBAD-available BV and ubvy colors on the one hand, and to 1993 Kurucz synthetic spectra on the other, we show our data to be accurate to 0.01 mag for the 13 passbands at or above 400 nm, and 0.02 mag for the 3 passbands below 400 nm. We also show that the scatter in the fits of the spectrophotometric colors and the uvby filter colors is a reasonable way to identify the observations of which specific stars are accurate to 1-sigma, 2-sigma, ... The very good agreement between the models and these data verifies the accuracy of these data, and also verifies the usefulness of the Kurucz models to define spectrophotometry for stars in this temperature range (>5000 K). These data define accurate spectrophotometry of bright, open cluster stars that can be used as a secondary flux calibration for CCD-based spectrophotometric surveys.

==> readadctables <==
%auto-ignore
J/AJ/000/000  Spectrophotometry of 237 stars in 7 Open Clusters
================================================================================
Spectrophotometry of 237 stars in 7 Open Clusters
         <Astronomical J. 00, 00 (1997)>
         =1997AJ...00...00T
================================================================================

Keywords: open clusters; open cluster stars --- spectrophotometry

Abstract:  

    Photoelectric spectrophotometry, normalized to the Hayes-Latham standard,
is given for stars in the Hyades, Pleiades, alpha Persei, Coma Berenices,
Praesepe, IC 4665 and M39.  The spectrophotometry consists of 16 filters of 
width 3.2-6.4 nm, normalized to 555.6 nm.  Comparison to available uvby and
UBV photometry, the 1993 synthetic models of Kurucz, and the spectrophotometry
of Adelman et al. indicate a one-sigma error per observation of 0.01 mag 
redward of 4.0 nm; and 0.02 mag blueward.

Introduction:

    The two major data tables in this paper are in ascii format, the
descriptions of which are contained in this README file.  

Table 4 gives the spectrophometry details.

Table 6 gives the related data for each star as obtained both by queries to
SIMBAD, as well as through comparison with Kurucz models.

File Summary:
--------------------------------------------------------------------------------
File Name            Lrecl        Records     Explanations
--------------------------------------------------------------------------------
ReadMe                  80              .     This file
table4                 125            237     16 Filter Spectrophotometry
table6                 131            237     SIMBAD, Kurucz Data, Comparisons
--------------------------------------------------------------------------------


Byte-by-byte Description of file: table4
--------------------------------------------------------------------------------
  Bytes Format  Units    Label     Explanations
--------------------------------------------------------------------------------
  2-  7  A7     ---      Starnum   Number for star (1)
  9- 13  A5     ---      Night     Nights observed (2)
 16- 19  I4     mag      3500      [9999]? 3500-5556 color (3)
 20      A1     ---      u_3500    [ ,:,*] indicates larger error in color (3)
 23- 26  I4     mag      3571      [9999]? 3571-5556 color (3)
 27      A1     ---      u_3571    [ ,:,*] indicates larger error in color (3)
 30- 33  I4     mag      3636      [9999]? 3636-5556 color (3)
 34      A1     ---      u_3636    [ ,:,*] indicates larger error in color (3)
 37- 40  I4     mag      4036      [9999]? 4036-5556 color (3)
 41      A1     ---      u_4036    [ ,:,*] indicates larger error in color (3)
 44- 47  I4     mag      4167      [9999]? 4167-5556 color (3)
 48      A1     ---      u_4167    [ ,:,*] indicates larger error in color (3)
 51- 54  I4     mag      4255      [9999]? 4255-5556 color (3)
 55      A1     ---      u_4255    [ ,:,*] indicates larger error in color (3)
 58- 61  I4     mag      4400      [9999]? 4400-5556 color (3)
 62      A1     ---      u_4400    [ ,:,*] indicates larger error in color (3)
 65- 68  I4     mag      4565      [9999]? 4565-5556 color (3)
 69      A1     ---      u_4565    [ ,:,*] indicates larger error in color (3)
 72- 75  I4     mag      4785      [9999]? 4785-5556 color (3)
 76      A1     ---      u_4785    [ ,:,*] indicates larger error in color (3)
 79- 82  I4     mag      5000      [9999]? 5000-5556 color (3)
 83      A1     ---      u_5000    [ ,:,*] indicates larger error in color (3)
 86- 89  I4     mag      5263      [9999]? 5263-5556 color (3)
 90      A1     ---      u_5263    [ ,:,*] indicates larger error in color (3)
 93- 96  I4     mag      5840      [9999]? 5840-5556 color (3)
 97      A1     ---      u_5840    [ ,:,*] indicates larger error in color (3)
100-103  I4     mag      6300      [9999]? 6300-5556 color (3)
104      A1     ---      u_6300    [ ,:,*] indicates larger error in color (3)
107-110  I4     mag      6710      [9999]? 6710-5556 color (3)
111      A1     ---      u_6710    [ ,:,*] indicates larger error in color (3)
114-117  I4     mag      7100      [9999]? 7100-5556 color (3)
118      A1     ---      u_7100    [ ,:,*] indicates larger error in color (3)
121-124  I4     mag      7400      [9999]? 7400-5556 color (3)
125      A1     ---      u_7400    [ ,:,*] indicates larger error in color (3)


--------------------------------------------------------------------------------
Note (1):
    Bytes 2-7 (Starnum) - Number of star according to the following sources:
       Hyades (Hya):         Van Bueren, 1952, B. A. N. 11, No. 432
       Pleiades (Ple):       Hertzsprung, E., 1947, Ann. Leiden Obs. 19, No. 1A
       alpha Per (Per):      Heckmann, O., Dieckvoss, W., \& Kox, H., 1956, 
                             A. N. 283, 109
       Praesepe (Pra):       Klein-Wassink, W. J., 1927, Groningen Publ. No. 41
       Coma Berenices (Com): Trumpler, F. J., 1938, Lick Obs. Bull. 18, 167
       IC 4665 (IC4):        Kopff, 1943, Mitt. Hamburg Stw. 8, 52
       M39 (M39):            Ebbinghausen, E. G., 1940, ApJ 92, 434

Note (2):
    Bytes 9-13 (Night) - Night of observation + secondary standard star(s)
                         used for night
      1   July 17/18, 1973   M39                           M39 33
      2   Aug. 14/15         Pleiades                      Ple 785
      3   Aug. 15/16         M39,alpha Persei              Per 605
      4   Sept. 15/16        Pleiades                      Ple 785
      5   Sept. 16/17        Hyades                        Hya 56
      6   Sept. 17/18        alpha Persei,Pleiades         Ple 785
      7   Sept. 18/19        Pleiades                      Ple 785
      8   Sept. 20/21        Hyades                        Hya 56
      9   Oct. 12/13         Hyades                        Hya 56
     10   Oct. 13/14         Hyades                        Hya 56
     11   Mar. 8/9, 1974     Hyades,Praesepe,Coma B.       Hya 56
     12   Mar. 9/10          Coma B.                       Com 60
     13   Apr. 10/11         Praesepe                      Pra 300
     14   May 6/7            Coma B.                       Com 60
     15   May 7/8            Praesepe,Coma B.,IC 4665      Pra 300,Com 60
     16   Aug. 9/10          IC 4665                       IC4 62
     17   Dec. 29/30         Hyades,Pleiades,alpha Persei  Hya 56
   stan   If star is used as secondary standard for that cluster

Note (3):
    Bytes (16-19),(23-26), ... - spectrophotometric colors of the cited filter
        formed with the 5556 filter (15 colors).  All colors are expressed
        in terms of magnitudes multiplied by 1000 (e.g., a color of 1225 is
        a color of 1.225 mag).
    Byte (20),(27), ... - indicator if error of observation known to be larger
        than typical error.  
        : = error of 0.03-0.06 mag; 
        * = interpolated value from star color and bracketing observations.
--------------------------------------------------------------------------------

Byte-by-byte Description of file: table6
--------------------------------------------------------------------------------
  Bytes Format  Units    Label     Explanations
--------------------------------------------------------------------------------
  1-  8  A8     ---      Starnum   Number for star (1)
 10- 15  I5     ---      HD_num    []=? HD number of star
 17- 18  I2     h        RAh       Right Ascension 1950 (hours) (2)
 20- 21  I2     min      RAm       Right Ascension 1950 (minutes) (2)
 23- 26  F4.1   s        RAs       Right Ascension 1950 (seconds) (2)
 27      A1     -        DE-       Declination 1950 (sign) (2)
 28- 29  I2     h        DEd       Declination 1950 (degrees) (2)
 31- 32  I2     arcmin   DEm       Declination 1950 (minutes) (2)
 34- 37  F4.1   arcsec   DEs       Declination 1950 (seconds) (2)
 39- 47  A9     ---      Sp        Spectral type from SIMBAD (2)
 49      A1     ---      Notes     Notes for particular stars (3)
 50- 54  F5.2   mag      V_mag     apparent V mag from SIMBAD
 56- 61  F6.3   mag      B-V       [9.999]=?, observed B-V color from SIMBAD
 64- 68  F5.3   mag      u-b       [9.999]=?, observed u-b color from SIMBAD
 71- 75  F5.3   mag      v-y       [9.999]=?, observed v-y color from SIMBAD
 77- 82  F6.3   mag      b-y       [9.999]=?, observed b-y color from SIMBAD
 85- 90  F6.3   mag      del_B-V   [9.999]=?, B-V color diff, US-SIMBAD (4)
 92- 97  F6.3   mag      del_u-b   [9.999]=?, u-b color diff, US-SIMBAD (4)
 98      A1     ---      e_delub   [ :], bad u-b color comparision (4)
 99-104  F6.3   mag      del_v-y   [9.999]=?, v-y color diff, US-SIMBAD (4)
105      A1     ---      e_delvy   [ :], bad v-y color comparision (4)
106-111  F6.3   mag      del_b-y   [9.999]=?, b-y color diff, US-SIMBAD (4)
112      A1     ---      e_delby   [ :], bad b-y color comparision (4)
113-118  F6.3   mag      d_kurbl   [9.999]=?, Kurucz comparison, blue col (5) 
120-125  F6.3   mag      d_kurrd   [9.999]=?, Kurucz comparison, red col (5) 
127-131  F5.2   mag      Abs_V     Absolute V mag (6)
--------------------------------------------------------------------------------
Note (1):
    Bytes 1-8 (Starnum) - See Note (1) for Table 4

Note (2):
    Right Ascension and Declination in 1950 coordinates as given by SIMBAD.
    Bytes 39-47 (Sp) is the spectral type from SIMBAD.  A colon on either
                spectral class or luminosity class indicates uncertainty.

Note (3):
    Byte 49 (Notes) - Data come from SIMBAD unless a note is given.  The note
                      code is:
       c = these stars are variable according to SIMBAD
       d = Luminosity class taken from Mendoza, E. E. 1967, 
           Bol Ton y Tac 4, 149
       e = Spectral class taken from Crawford, D. L. \& Barnes, J. V. 
           1972, AJ 77, 862
       f = Luminosity class taken from Crawford & Barnes

Note (4):
    Bytes 85-90 (del_B-V), 92-97 (del_u-b), 
          99-104 (del_v-y), 106-111 (del_b-y) 
          - The residuals from comparing the spectrophotometric colors with
            B-V, u-b, v-y, b-y colors from SIMBAD.  The color transformations
            are as follows:
           Color  Transformation             Slope   Z.P.    error
  Johnson    B-V  Matthews & Sandage (1963)  1.072   0.433   0.021
  Stromgren  u-b  3500 - (4565+4785)/2       1.005   0.125   0.024
  Stromgren  b-y  (4565+4785)/2              0.934   0.153   0.013
  Stromgren  v-y  (4036+4167)/2              0.891   0.415   0.032
           The color transformation for B-V was done using the airmass = 1
           bandpass functions for B and V mag as given by Matthews & Sandage

    Byte 98 (e_delub), 105 (e_delvy), 112 (e_delby)
           - If indicated by a colon (:), this color comparison was
             not used in determining the color transformations.

Note (5): 
     Bytes 113-118 (d_kurbl) and 120-125 (d_kurrd)
           - These are the average residuals from the best fit of Kurucz
             main sequence model spectral energy distributions to the main 
             sequence stars in our sample.  d_kurbl are the residuals for
             the three colors with one passband falling below 4000 angstroms.
             d_kurrd are the residuals for the 12 colors with both passbands
             falling at or above 4000 angstroms.

     Note that the residuals from the Kurucz fit (d_kurbl and d_kurrd) are
well-correlated with the residuals from the uvby fits (d_kurbl with del_u-b;
d_kurrd with del_b-y), so that the size of the color residuals is a good 
indication of the error of spectrophotometric observation, as detailed in
the paper.

Note (6):
     Bytes 127-131 (Abs_V) - The absolute V magnitude, extinction corrected,
        according to the following values for reddening and distances:
                       dist(pc)  E(B-V)
        Praesepe         180     0.03
        Hyades            43     0.00
        Coma Berenices    90     0.00
        M39              290     0.06
        Pleiades         180     0.06
        IC 4665          470     0.17
        alpha Persei     230     0.10
        The distances are estimated by a direct fit of the ZAMS line from
        Mihalas & Binney (1981, Freeman) to the V vs. B-V diagrams as
        published in our paper.  The reddenings come from the 5th edition
        of the Lund-Strasbourg Catalog (Lynga 1987)
-------------------------------------------------------------------------------

================================================================================
(End)     D. Burstein/L. Clampitt       [ASU]                        May-19-1997

